A Gaussian Process Model for Opponent Prediction in Autonomous Racing

In head-to-head racing, an accurate model of interactive behavior of the opposing target vehicle (TV) is required to perform tightly constrained, but highly rewarding maneuvers such as overtaking. However, such information is not typically made available in competitive scenarios, we therefore propose to construct a prediction and uncertainty model given data of the TV from previous races. In particular, a one-step Gaussian process (GP) model is trained on closed-loop interaction data to learn the behavior of a TV driven by an unknown policy. Predictions of the nominal trajectory and associated uncertainty are rolled out via a sampling-based approach and are used in a model predictive control (MPC) policy for the ego vehicle in order to intelligently trade-off between safety and performance when attempting overtaking maneuvers against a TV. We demonstrate the GP-based predictor in closed loop with the MPC policy in simulation races and compare its performance against several predictors from literature. In a Monte Carlo study, we observe that the GP-based predictor achieves similar win rates while maintaining safety in up to 3x more races. We finally demonstrate the prediction and control framework in real-time in a experimental study on a 1/10th scale racecar platform operating at speeds of around 2.8 m/s, and show a significant level of improvement when using the GP-based predictor over a baseline MPC predictor. Videos of the hardware experiments can be found at https://youtu.be/KMSs4ofDfIs.

==> notes.tex <==
abstract

Section 1:

Section 2:
- Jake and Finn read through and give feedback

Section 3:
- Jake and Finn read through and give feedback
- Could possibly use a couple of examples of simulation rollouts

Section 4:
- rearrange v_x

Section 5:
- Section 5C when discussing the prediction accuracy, should use numbers for mean squared error and error standard deviation.
- merge pred accuracy with closed loop
- For the experiments track, let's show a frame of the video with the track and some history overlaid on top
- Wins/crash rate explanation
- Experimental validation with current hardware experiments

